Random walk kernels and learning curves for Gaussian process regression on random graphs

We consider learning on graphs, guided by kernels that encode similarity between vertices. Our focus is on random walk kernels, the analogues of squared exponential kernels in Euclidean spaces. We show that on large, locally treelike, graphs these have some counter-intuitive properties, specifically in the limit of large kernel lengthscales. We consider using these kernels as covariance matrices of e.g.\ Gaussian processes (GPs). In this situation one typically scales the prior globally to normalise the average of the prior variance across vertices. We demonstrate that, in contrast to the Euclidean case, this generically leads to significant variation in the prior variance across vertices, which is undesirable from the probabilistic modelling point of view. We suggest the random walk kernel should be normalised locally, so that each vertex has the same prior variance, and analyse the consequences of this by studying learning curves for Gaussian process regression. Numerical calculations as well as novel theoretical predictions for the learning curves using belief propagation make it clear that one obtains distinctly different probabilistic models depending on the choice of normalisation. Our method for predicting the learning curves using belief propagation is significantly more accurate than previous approximations and should become exact in the limit of large random graphs.

==> figs/gnuplot/appscaling.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(8616.00,4308.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{} 0}}%
      \put(946,1008){\makebox(0,0)[r]{\strut{} 0.2}}%
      \put(946,1311){\makebox(0,0)[r]{\strut{} 0.4}}%
      \put(946,1615){\makebox(0,0)[r]{\strut{} 0.6}}%
      \put(946,1918){\makebox(0,0)[r]{\strut{} 0.8}}%
      \put(946,2222){\makebox(0,0)[r]{\strut{} 1}}%
      \put(946,2525){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(946,2829){\makebox(0,0)[r]{\strut{} 1.4}}%
      \put(946,3132){\makebox(0,0)[r]{\strut{} 1.6}}%
      \put(946,3436){\makebox(0,0)[r]{\strut{} 1.8}}%
      \put(946,3739){\makebox(0,0)[r]{\strut{} 2}}%
      \put(946,4043){\makebox(0,0)[r]{\strut{} 2.2}}%
      \put(1078,484){\makebox(0,0){\strut{} 0}}%
      \put(2863,484){\makebox(0,0){\strut{} 0.5}}%
      \put(4649,484){\makebox(0,0){\strut{} 1}}%
      \put(6434,484){\makebox(0,0){\strut{} 1.5}}%
      \put(8219,484){\makebox(0,0){\strut{} 2}}%
      \put(176,2373){\rotatebox{-270}{\makebox(0,0){\strut{}$p\rho_{l,p}$}}}%
      \put(4648,154){\makebox(0,0){\strut{}$l/p^{1/2}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figs/gnuplot/appscaling}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figs/gnuplot/mismatch.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(8640.00,4320.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(528,704){\makebox(0,0)[r]{\strut{}$10^{-2}$}}%
      \put(528,2380){\makebox(0,0)[r]{\strut{}$10^{-1}$}}%
      \put(528,4055){\makebox(0,0)[r]{\strut{}$10^{0}$}}%
      \put(660,484){\makebox(0,0){\strut{}$10^{-2}$}}%
      \put(1476,484){\makebox(0,0){\strut{}$10^{-1}$}}%
      \put(2292,484){\makebox(0,0){\strut{}$10^{0}$}}%
      \put(3108,484){\makebox(0,0){\strut{} }}%
      \put(-242,2379){\rotatebox{-270}{\makebox(0,0){\strut{}$\epsilon$}}}%
      \put(1884,154){\makebox(0,0){\strut{} }}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1581,1765){\makebox(0,0)[r]{\strut{}$\sigma^{2} = 10^{-1}$}}%
      \csname LTb\endcsname%
      \put(1581,1545){\makebox(0,0)[r]{\strut{}$\sigma^{2} = 10^{-2}$}}%
      \csname LTb\endcsname%
      \put(1581,1325){\makebox(0,0)[r]{\strut{}$\sigma^{2} = 10^{-3}$}}%
      \csname LTb\endcsname%
      \put(1581,1105){\makebox(0,0)[r]{\strut{}$\sigma^{2} = 10^{-4}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(2979,704){\makebox(0,0)[r]{\strut{}}}%
      \put(2979,2380){\makebox(0,0)[r]{\strut{}}}%
      \put(2979,4055){\makebox(0,0)[r]{\strut{}}}%
      \put(3111,484){\makebox(0,0){\strut{}$10^{-2}$}}%
      \put(3974,484){\makebox(0,0){\strut{}$10^{-1}$}}%
      \put(4837,484){\makebox(0,0){\strut{}$10^{0}$}}%
      \put(5700,484){\makebox(0,0){\strut{}$10^{1}$}}%
      \put(4405,154){\makebox(0,0){\strut{}$\nu=N/V$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(6272,2378){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(6272,2697){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \put(6272,3017){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(6272,3336){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \put(6272,3656){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \put(6272,3975){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(5326,3216){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \put(7059,2312){\makebox(0,0){\strut{}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(6272,704){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(6272,1022){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \put(6272,1340){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(6272,1658){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \put(6272,1976){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \put(6272,2294){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(6008,484){\makebox(0,0){\strut{}$10^{-2}$}}%
      \put(6797,484){\makebox(0,0){\strut{}$10^{-1}$}}%
      \put(7586,484){\makebox(0,0){\strut{}$10^{0}$}}%
      \put(8375,484){\makebox(0,0){\strut{}$10^{1}$}}%
      \put(5326,1538){\rotatebox{-270}{\makebox(0,0){\strut{}}}}%
      \put(7059,154){\makebox(0,0){\strut{} }}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{figs/gnuplot/mismatch}}%
    \gplfronttext
  \end{picture}%
\endgroup

